SelfGNN: Self-Supervised Graph Neural Networks for Sequential Recommendation

Sequential recommendation effectively addresses information overload by modeling users' temporal and sequential interaction patterns. To overcome the limitations of supervision signals, recent approaches have adopted self-supervised learning techniques in recommender systems. However, there are still two critical challenges that remain unsolved. Firstly, existing sequential models primarily focus on long-term modeling of individual interaction sequences, overlooking the valuable short-term collaborative relationships among the behaviors of different users. Secondly, real-world data often contain noise, particularly in users' short-term behaviors, which can arise from temporary intents or misclicks. Such noise negatively impacts the accuracy of both graph and sequence models, further complicating the modeling process. To address these challenges, we propose a novel framework called Self-Supervised Graph Neural Network (SelfGNN) for sequential recommendation. The SelfGNN framework encodes short-term graphs based on time intervals and utilizes Graph Neural Networks (GNNs) to learn short-term collaborative relationships. It captures long-term user and item representations at multiple granularity levels through interval fusion and dynamic behavior modeling. Importantly, our personalized self-augmented learning structure enhances model robustness by mitigating noise in short-term graphs based on long-term user interests and personal stability. Extensive experiments conducted on four real-world datasets demonstrate that SelfGNN outperforms various state-of-the-art baselines. Our model implementation codes are available at https://github.com/HKUDS/SelfGNN.

==> figure/hyper2.tex <==
\begin{tikzpicture}
\begin{axis}[
    width=12cm, % 设置图像宽度
    height=8cm, % 设置图像高度
    xlabel={Number of Short-term Graphs $T$},
    ylabel={Decrease of nDCG@10 (\%)},
    xmin=2,xmax=7,
    ymin=-40,ymax=5,
    legend columns=1,
    legend cell align=right,
    grid=both,
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=1.3},
    label style={scale=1.8},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(1,0)},anchor=south east},
    every axis plot post/.append style={
        every mark/.append style={scale=2}
    }
]
\addplot[color={rgb:red,133;green,76;blue,255}, mark=o, mark options={solid}]
table[x=para, y=gowalla_ndcg] {latFactor.txt};
\addplot[color={rgb:red,0;green,157;blue,178}, mark=square, mark options={solid}]
table[x=para, y=ml10m_ndcg] {latFactor.txt};
\addplot[color={rgb:red,245;green,9;blue,11}, mark=triangle, mark options={solid}]
table[x=para, y=amazon_ndcg] {latFactor.txt};
\addplot[color={rgb:red,10;green,10;blue,240}, mark=x, mark options={solid}]
table[x=para, y=yelp_ndcg] {latFactor.txt};
\legend{\large Gowalla, \large MovieLens, \large Amazon, \large Yelp};
\end{axis}
% Add a second x-axis at the top
\begin{axis}[
    width=12cm, % 设置图像宽度
    height=8cm, % 设置图像高度
xmin=4,xmax=14,
ymin=-40,ymax=5,
axis x line=top,
axis y line=none,
xlabel={Number of Short-term Graphs $T$ for Yelp},
ylabel={}
]
\end{axis}
\end{tikzpicture}


\begin{tikzpicture}
\begin{axis}[
    width=12cm, % 设置图像宽度
    height=8cm, % 设置图像高度
    xlabel={User Personalized Weight $d_{sal}$},
    ylabel={Decrease of nDCG@10 (\%)},
    xmin=16,xmax=48,
    ymin=-15,ymax=1,
    legend columns=1,
    legend cell align=right,
    grid=both,
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=1.3},
    label style={scale=1.8},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(1,0)},anchor=south east},
    every axis plot post/.append style={
        every mark/.append style={scale=2}
    }
]
\addplot[color={rgb:red,133;green,76;blue,255}, mark=o, mark options={solid}]
table[x=para, y=gowalla_ndcg] {hyperNum.txt};
\addplot[color={rgb:red,0;green,157;blue,178}, mark=square, mark options={solid}]
table[x=para, y=ml10m_ndcg] {hyperNum.txt};
\addplot[color={rgb:red,245;green,9;blue,11}, mark=triangle, mark options={solid}]
table[x=para, y=amazon_ndcg] {hyperNum.txt};
\addplot[color={rgb:red,10;green,10;blue,240}, mark=x, mark options={solid}]
table[x=para, y=yelp_ndcg] {hyperNum.txt};
\legend{\large Gowalla, \large MovieLens, \large Amazon, \large Yelp};
\end{axis}
\end{tikzpicture}




==> figure/hyper3.tex <==


\begin{tikzpicture}
\begin{axis}[
    width=12cm, % 设置图像宽度
    height=8cm, % 设置图像高度
    xlabel={Weight for SAL Loss $\lambda_1$ ($1e^{-x}$)},
    ylabel={Decrease of HR@10 (\%)},
    xmin=4,xmax=7,
    ymin=-30,ymax=1,
    legend columns=1,
    legend cell align=right,
    grid=both,
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=1.3},
    label style={scale=1.8},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(1,0)},anchor=south east},
    every axis plot post/.append style={
        every mark/.append style={scale=2}
    }
]
\addplot[color={rgb:red,133;green,76;blue,255}, mark=o, mark options={solid}]
table[x=para, y=gowalla_hr] {lamda.txt};
\addplot[color={rgb:red,0;green,157;blue,178}, mark=square, mark options={solid}]
table[x=para, y=ml10m_hr] {lamda.txt};
\addplot[color={rgb:red,245;green,9;blue,11}, mark=triangle, mark options={solid}]
table[x=para, y=amazon_hr] {lamda.txt};
\addplot[color={rgb:red,10;green,10;blue,240}, mark=x, mark options={solid}]
table[x=para, y=yelp_hr] {lamda.txt};
\legend{\large Gowalla, \large MovieLens, \large Amazon, \large Yelp};
\end{axis}
\end{tikzpicture}



\begin{tikzpicture}
\begin{axis}[
    width=12cm, % 设置图像宽度
    height=8cm, % 设置图像高度
    xlabel={Number of Edge-pairs Samples $N_{sal}$},
    ylabel={Decrease of HR@10 (\%)},
    xmin=20,xmax=100,
    ymin=-12,ymax=2,
    legend columns=1,
    legend cell align=right,
    grid=both,
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=1.3},
    label style={scale=1.8},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(1,0)},anchor=south east},
    every axis plot post/.append style={
        every mark/.append style={scale=2}
    }
]
\addplot[color={rgb:red,133;green,76;blue,255}, mark=o, mark options={solid}]
table[x=para, y=gowalla_hr] {sampnum.txt};
\addplot[color={rgb:red,0;green,157;blue,178}, mark=square, mark options={solid}]
table[x=para, y=ml10m_hr] {sampnum.txt};
\addplot[color={rgb:red,245;green,9;blue,11}, mark=triangle, mark options={solid}]
table[x=para, y=amazon_hr] {sampnum.txt};
\addplot[color={rgb:red,10;green,10;blue,240}, mark=x, mark options={solid}]
table[x=para, y=yelp_hr] {sampnum.txt};
\legend{\large Gowalla, \large MovieLens, \large Amazon, \large Yelp};
\end{axis}
\end{tikzpicture}

==> figure/hyper4.tex <==
\begin{tikzpicture}
\begin{axis}[
    width=12cm, % 设置图像宽度
    height=8cm, % 设置图像高度
    xlabel={Weight for SAL Loss $\lambda_1$ ($1e^{-x}$)},
    ylabel={Decrease of nDCG@10 (\%)},
    xmin=4,xmax=7,
    ymin=-30,ymax=1,
    legend columns=1,
    legend cell align=right,
    grid=both,
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=1.3},
    label style={scale=1.8},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(1,0)},anchor=south east},
    every axis plot post/.append style={
        every mark/.append style={scale=2}
    }
]
\addplot[color={rgb:red,133;green,76;blue,255}, mark=o, mark options={solid}]
table[x=para, y=gowalla_ndcg] {lamda.txt};
\addplot[color={rgb:red,0;green,157;blue,178}, mark=square, mark options={solid}]
table[x=para, y=ml10m_ndcg] {lamda.txt};
\addplot[color={rgb:red,245;green,9;blue,11}, mark=triangle, mark options={solid}]
table[x=para, y=amazon_ndcg] {lamda.txt};
\addplot[color={rgb:red,10;green,10;blue,240}, mark=x, mark options={solid}]
table[x=para, y=yelp_ndcg] {lamda.txt};
\legend{\large Gowalla, \large MovieLens, \large Amazon, \large Yelp};
\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[
    width=12cm, % 设置图像宽度
    height=8cm, % 设置图像高度
    xlabel={Number of Edge-pairs Samples $N_{sal}$},
    ylabel={Decrease of nDCG@10 (\%)},
    xmin=20,xmax=100,
    ymin=-12,ymax=2,
    legend columns=1,
    legend cell align=right,
    grid=both,
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=1.3},
    label style={scale=1.8},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(1,0)},anchor=south east},
    every axis plot post/.append style={
        every mark/.append style={scale=2}
    }
]
\addplot[color={rgb:red,133;green,76;blue,255}, mark=o, mark options={solid}]
table[x=para, y=gowalla_ndcg] {sampnum.txt};
\addplot[color={rgb:red,0;green,157;blue,178}, mark=square, mark options={solid}]
table[x=para, y=ml10m_ndcg] {sampnum.txt};
\addplot[color={rgb:red,245;green,9;blue,11}, mark=triangle, mark options={solid}]
table[x=para, y=amazon_ndcg] {sampnum.txt};
\addplot[color={rgb:red,10;green,10;blue,240}, mark=x, mark options={solid}]
table[x=para, y=yelp_ndcg] {sampnum.txt};
\legend{\large Gowalla, \large MovieLens, \large Amazon, \large Yelp};
\end{axis}
\end{tikzpicture}

==> model_back.tex <==
\section{Preliminaries and Related Work}
\label{sec:model}
\subsection{Graph Neural Network for Recommendation}
Recent studies have attempted to design a variety of GNN architectures to seek the display and implicit correlation. One mainstream direction is capturing high-order CF signals with multi-hop interaction topological structures such as NGCF \cite{NGCF} and SGL \cite{SGL}, then efficiency is further improved by LightGCN \cite{LightGCN} which omits the non-linear transformation in GCN. On the other side, SRGNN \cite{SRGNN} and GCE-GNN \cite{GCE-GNN} separate session sequences into graph-structured data. SURGE \cite{SURGE} processes item-item sequential graphs through metric learning and uses cluster-aware GCNs to dynamically extract the users' interests. %CF signals lie in that the more similar the historical behavior the more likely the users share similar interests.

Despite the remarkable success, most methods lack consideration of the noise in the graphs and the temporal and dynamic characteristics of the CF graphs \cite{Huang_2021}. Hence, we obtain periodical user-item relationships by dividing the global graph into many short-term graphs according to the time interval, fusing the short-term features into long interests with attentive sequence modeling, and introducing a self-augmented signal to mitigate noise from the sparse short-term graphs. Specifically, we define $\mathcal{U}=\{u_1,...,u_i,...,u_I\}(|\mathcal{U}|=I)$ and $\mathcal{V}=\{v_1,...,v_j,...,v_J\}$ $(|\mathcal{V}|=J)$ to represent the set of users and items respectively. We divide the dataset equally into $T$ periods from the earliest interaction time to the latest time in it. The adjacent matrix $\mathcal{A}_t\in \mathbb{R}^{I\times J}$ indicates the implicit relationships between each user and the items they interacted with in the ($t$)-th period, every entry $\mathcal{A}_{t,i,j}$ in $\mathcal{A}_{t}$ will be set as 1 if the user $u_{i}$ has adopted the item $v_j$ and $\mathcal{A}_{t,i,j}=0$ otherwise.

\subsection{Sequential Recommender System}
The sequence indicates an ordered list of user actions \cite{yang2022multi}. There are strong sequential dependencies between objects within a sequence. Several models have focused on the time-evolving user preference, \eg, session recommendations with RNNs (GRU4Rec \cite{GRU4Rec}). Owing to the strength of the Transformer framework, self-attention has been widely used to capture the item-item correlations in SASRec \cite{SASRec}, Bert4Rec \cite{Bert4Rec} and TiSASRec \cite{TiSASRec} with time interval aware. Furthermore, SASRec has been improved by ICLRec \cite{ICLRec} with cluster method to learn users' intentions. In our work, we innovatively propose to combine higher-order collaborative graphs with sequence information. In particular, the sequences of period granularity composed of short-term graphs are combined with instance-level sequences of user behavior to achieve multi-level sequential modeling in our \model\ framework.

\subsection{Self-Supervised Learning}
As self-supervised learning provides auxiliary signals \cite{Liu_2021}, it plays an essential role in improving the embedding quality of supervised learning. In graph recommendation, SGL \cite{SGL} takes node self-discrimination to mitigate bias and increase robustness, CoTRec \cite{CoTRec} performs bi-level contrastive learning by building two homogeneous graphs from item and session perspectives. In addition, HCCF \cite{HCCF} integrates hypergraph encoding with self-supervised learning. In the sequential scenario, ICLRec \cite{ICLRec} and CoSeRec \cite{CoSeRec} construct contrastive learning between sequences augmented by cropping, masking, or recording. Unlike them, this work proposes personalized augmented learning between the edges in short and long-term graphs, enhancing the short-term embedding learning.


==> relate.tex <==
\section{Related Work}
\label{sec:relate}

==> solution_back.tex <==
\section{Methodology}
\label{sec:solution}

\begin{figure*}
\centering
\includegraphics[width=16cm,angle=0]{figure/SLSG-framework.pdf}
\caption{Overall framework of the proposed \model\ model.} 
\label{fig:overall}
\end{figure*}
We introduce our proposed \model\ framework and illustrate the overall model architecture in Figure \ref{fig:overall}. \textit{First}, we utilize GNNs to obtain embedding vectors for users and items in each short-term graph. \textit{Second}, the long-term user interests are derived from a two-level sequential learning approach. \textit{Finally}, we introduce a personalized self-augmented learning architecture that combines long and short-term features to mitigate the impact of noise. %Second, we leverage the multi-head self-attention to capture the characteristics of users and items and their changing trends based on short-term embedding fusion and long-term sequential learning.The main notation used in our work is provided in the Appendix. 
\subsection{Short-term Collaborative Relation Encoding}
In order to capture the dynamic collaborative relationship between users and items, we split the long-term user behavior into $T$ short-term subgraphs in chronological order, and every subgraph uses GNNs to learn the embedding vectors ${\mathbf{e}_t^{(u)}}_i\in \mathbb{R}^{d}$ for user $u_i$ and ${\mathbf{e}_t^{(v)}}_j\in \mathbb{R}^{d}$ for item $v_j$ in a $d$-dimensional latent space, in which $t$ means the embedding from period $t$. Also, in each period $t$, we aggregate all the user and item embeddings to compose embedding matrices $\mathbf{E}_t^{(u)} \in \mathbb{R}^{I\times d}$ and $\mathbf{E}_t^{(v)} \in \mathbb{R}^{J\times d}$ respectively. Inspired by LightGCN \cite{LightGCN}, we design our short-term graph layer as follows: %an effective GNN paradigm in information propagation, \mathbf{E}^{(u)} \in \mathbb{R}^{ T \times I\times d}$ and $\mathbf{E}^{(v)} \in \mathbb{R}^{T \times J\times d}$
\begin{equation}{\mathbf{z}_t^{(u)}}_i=\sigma( {\mathcal{A}_t}_{i,*}\cdot \mathbf{E}_t^{(v)}), {\mathbf{z}_t^{(v)}}_j=\sigma( {\mathcal{A}_t}_{j,*}\cdot \mathbf{E}_t^{(u)})\end{equation}
where ${\mathbf{z}_t^{(u)}}_i,{\mathbf{z}_t^{(v)}}_j\in \mathbb{R}^{d}$ denote the information aggregated by the short-term binary graph from neighboring nodes to the centric node $u_i$ and $v_j$. $\mathcal{A}_t$ represents the binary adjacent matrix in period ($t$)-th and $\sigma(\cdot)$ denotes the LeakyReLU activate function, which brings non-linearity to the transformation. It is worth mentioning that we adopt a random drop operation to the edges of the graphs to improve the robustness and mitigate the overfitting problem. % \in \mathbb{R}^{I \times J}

In addition, we stack several layers of GNNs to achieve high-order message propagation. In the $(l)$-th step, the message-passing process is formulated as:
\begin{equation}{\mathbf{e}_t^{(u)}}_{i,l}={\mathbf{z}_t^{(u)}}_{i,l}+{\mathbf{e}_t^{(u)}}_{i,l-1},{\mathbf{e}_t^{(v)}}_{j,l}={\mathbf{z}_t^{(v)}}_{j,l}+{\mathbf{e}_t^{(v)}}_{j,l-1}\end{equation}
where ${\mathbf{e}_t^{(u)}}_{i,l}$ and ${\mathbf{e}_t^{(v)}}_{j,l}$ represent the embedding of $u_i$ and $v_j$ at the $(l)$-th GNN layer. In this way, we not only generate high-order contextual information but also alleviate the over-smoothing problem.

Since different layers emphasize different relations between nodes, which will make different contributions to the users and items feature learning, we concatenate representations from different layers to obtain the final short-term embedding:
\begin{equation}{\mathbf{e}_t^{(u)}}_{i}={\mathbf{e}_t^{(u)}}_{i,1}||\cdot \cdot \cdot ||{\mathbf{e}_t^{(u)}}_{i,l}, {\mathbf{e}_t^{(v)}}_{j}={\mathbf{e}_t^{(v)}}_{j,1}||\cdot \cdot \cdot ||{\mathbf{e}_t^{(v)}}_{j,L}\end{equation}
\subsection{Multi-level Long-term Sequential Learning}
After the short-term collaborative relation encoding, we aim to characterize the long-term relationship between users and items on two levels: i) Interval-Level Sequential Pattern Modeling, which integrates the short-term features into a long-term representation based on a temporal attention model, capturing the dynamic changes in different periods, and ii) Instance-Level Sequential Pattern Modeling, which uses a simple attention module for learning the complete long-term user behavior sequence, complemented with the features obtained from i) as multi-view learning.
\label{sec:interval-level}
\subsubsection{\bf Interval-Level Sequential Pattern Modeling}
% Short-term Feature Fusion based on Temporal Attention
Firstly, for every user and item, we construct the short-term features for different periods into a sequence,\eg, $u_i$'s interest changes is $\{{\mathbf{e}_1^{(u)}}_{i},{\mathbf{e}_2^{(u)}}_{i},...,{\mathbf{e}_T^{(u)}}_{i}\}$ and sequence of $v_j$'s feature changes is $\{{\mathbf{e}_1^{(v)}}_{j},{\mathbf{e}_2^{(v)}}_{j},...,{\mathbf{e}_T^{(v)}}_{j}\}$. Since the pure attention mechanism can only learn the relationship between interval and interval, which does not introduce the order or position information, we utilize the hidden state of the Gated Recurrent Unit (GRU) network \cite{an-etal-2019-neural} to make the features of interest for each period imply temporal information and update the features for each period to be a combination of features from the initial time to the ($t$)-th period, which will respond to time-based changes in features, rather than isolated features in this short period.
%\begin{equation}{\mathbf{r}_{gru}}_t=\Phi(\mathbf{W}_r[{\mathbf{h}_{gru}}_{t-1},\mathbf{e}_t])\end{equation}
%\begin{equation}{\mathbf{z}_{gru}}_t=\Phi(\mathbf{W}_z[{\mathbf{h}_{gru}}_{t-1},\mathbf{e}_t])\end{equation}
%\begin{equation}\tilde{\mathbf{h}_{gru}}_t=\rm{ tanh}(\mathbf{W}_{\tilde{h_{gru}}}[{\mathbf{r}_{gru}}_t\odot {\mathbf{h}_{gru}}_{t-1},\mathbf{e}_t])\end{equation}
%\begin{equation}{\mathbf{h}_{gru}}_t={\mathbf{z}_{gru}}_t\odot \mathbf{h}_t+(1-{\mathbf{z}_{gru}}_t)\odot \tilde{\mathbf{h}_{gru}}_t\end{equation}
%where $\mathbf{W}_r,\mathbf{W}_z,\mathbf{W}_{\tilde{h}}$ are the parameters of GRU, $\Phi (\cdot)$ denotes the sigmoid activation function and
\begin{equation}{{\mathbf{h}_{gru}}_t^{(u)}}_i=\mathrm{GRU}({\mathbf{e}_t^{(u)}}_{i},{{\mathbf{h}_{gru}}_{t-1}^{(u)}}_i)\end{equation}
\begin{equation}{{\mathbf{h}_{gru}}_t^{(v)}}_j=\mathrm{GRU}({\mathbf{e}_t^{(v)}}_{j},{{\mathbf{h}_{gru}}_{t-1}^{(v)}}_j)\end{equation}
We take the hidden state ${\mathbf{h}_{gru}}_t$ as a new sequence of feature changes: \begin{equation}{\mathbf{S}_{h}}_i^{(u)}=\{{{\mathbf{h}_{gru}}_1^{(u)}}_{i},{{\mathbf{h}_{gru}}_2^{(u)}}_{i},...,{{\mathbf{h}_{gru}}_T^{(u)}}_{i}\}\end{equation}
\begin{equation}{\mathbf{S}_{h}}_j^{(v)}=\{{{\mathbf{h}_{gru}}_1^{(v)}}_{j},{{\mathbf{h}_{gru}}_2^{(v)}}_{j},...,{{\mathbf{h}_{gru}}_T^{(v)}}_{j}\}\end{equation}
 Nextly, employing a multi-head self-attention mechanism \cite{vaswani2017attention} enables the model to obtain mutual relations and assign higher weights to more significant short-term CF information.
 \begin{equation} {\mathbf{h}_{t}^{(u)}}_i=\mathrm{MultiheadSelfAttention}({\mathbf{S}_{h}}_i^{(u)}) \end{equation}
  \begin{equation} {\mathbf{h}_{t}^{(v)}}_j=\mathrm{MultiheadSelfAttention}({\mathbf{S}_{h}}_j^{(v)}) \end{equation}
 %\begin{equation}\alpha_{t_1,t_2}^k=\frac{{\rm{exp}}({\mathbf{h}_{gru}}_{t_1}^T\mathbf{Q}_k{\mathbf{h}_{gru}}_{t_2})}{\sum_{t=1}^{T}{\rm{exp}}({{\mathbf{h}}_{gru}}_{t_1}^T\mathbf{Q}_k{{\mathbf{h}}_{gru}}_{t})}\end{equation}
%$$\begin{equation}\mathbf{h}_{t_1,k}=\mathbf{V}_k(\frac{\sum_{t_2=1}^{T}\alpha_{t_1,t_2}^k\mathbf{r}_{t_2}}{\sqrt{d_h}})\end{equation}
%\begin{equation}\mathbf{h}_{t_1}=\mathbf{h}_{t_1,1}||\cdot \cdot \cdot ||\mathbf{h}_{t_1,H}\end{equation}
 %where $\mathbf{h}_{k}$ is ($k$)-th self-attention head, $\mathbf{Q}_k$ and $\mathbf{V}_k$ are parameters of the ($k$)-th self-attention head, the total head number is noted as $H$, $d_h=d/H$, and $\alpha_{t_1,t_2}^k$ represents the relative importance between the ($t_1$)-th and ($t_2$)-th short-term feature changes embedding. 
 Finally, we sum up the features to obtain a long-term user embedding vector and the same to a long-term item embedding vector:

\begin{equation}{\mathbf{e}_{long term}^{(u)}}_i=\sum_{t=1}^T{\mathbf{h}_{t}^{(u)}}_i,{\mathbf{e}_{long term}^{(v)}}_j=\sum_{t=1}^T{\mathbf{h}_{t}^{(v)}}_j\label{evl}\end{equation}

\subsubsection{\bf Instance-Level Sequential Pattern Modeling}
% Long-term user Behaviour Sequence Modeling based on Attention
Motivated by the strength of the Transformer in sequence learning, we denote the sequence of behaviors of any user as $s=\{s_1,s_2,...,s_M\}$, where $M$ represents the maximum length and $s_m$ is the ($m$)-th item the user used to interact with. We further define $\mathbf{E}_{long term}^{(v)}\in \mathbb{R}^{J\times d}, \mathbf{E}_{long term}^{(v)}=\{{\mathbf{e}_{long term}^{(v)}}_1,...,{\mathbf{e}_{long term}^{(v)}}_J\}$ to represent the long-term item embedding and create a learnable position matrix $\mathbf{P}\in\mathbb{R}^{M\times d}$. Input the position encoding and the item sequence composed of the long-term item embeddings we just obtained into the multi-layer residual multi-head self-attention module: % according to Eq. \eqref{evl}
\begin{equation}\mathbf{S}_{instance}^0=[{\mathbf{E}_{long term}^{(v)}}_{s_1}+\mathbf{P}_1,...,{\mathbf{E}_{long term}^{(v)}}_{s_M}+\mathbf{P}_M]\end{equation}
%$${\rm{ATT}}(\mathbf{Q},\mathbf{K},\mathbf{V})=s(\frac{\mathbf{Q}\mathbf{K}}{\sqrt{d}})\mathbf{V}$$
%$$\mathbf{head}_k={\rm{ATT}}(\mathbf{Q}\W_k^Q,\mathbf{K}\W_k^K,\mathbf{V}\W_k^V)$$
%$${\rm{MHATT}}(\mathbf{Q},\mathbf{K},\mathbf{V})=\mathbf{head}_1||\cdot \cdot \cdot ||\mathbf{head}_{h}$$
%\begin{equation}{\rm{SA}}(\mathbf{S})={\rm{MHATT}}(\mathbf{S}\mathbf{W}^Q,\mathbf{S}\mathbf{W}^K,\mathbf{S}\mathbf{W}^V)\end{equation}
\begin{equation}\mathbf{S}_{instance}^{l}={\sigma}(\mathrm{MultiheadSelfAttention}(\mathbf{S}_{instance}^{l-1}))+\mathbf{S}_{instance}^{l-1} \label{al}\end{equation}
where Eq. \eqref{al} is the method for stacking $L_{att}$ layers of residual multi-head self-attention mechanisms. In the same way, we can obtain a long-term sequential interest profile for any user $i$, which has the long-term basic sequence information:
\begin{equation}{\e_{sequence}^{(u)}}_i={\mathbf{S}_{instance}^{L_{att}}}_i\end{equation} 
It is important to note that solely modeling long-term user behavior using the attention approach neglects high-order information and dynamic feature changes. Therefore, the fusion of features from different short-term intervals, as mentioned in Section \ref{sec:interval-level}, becomes crucial. This fusion enables multi-level user profile learning, which incorporates both the interval and instance-level components.

\subsection{Multi-view Aggregation and Prediction}
Before prediction, we aggregate the multi-views user features derived from the instance-level and the instance-level approach:
\begin{equation}{\e_{final}^{(u)}}_i={\e_{longterm}^{(u)}}_i+{\e_{sequence}^{(u)}}_i\label{eq:efinal}\end{equation}
%If the similarity is high, the probability that the user will be interested in the item will be high. Our main task is to make the model capable of outputting higher scores for positive samples than for negative ones based on the user behavior history.
When predicting the likelihood of an interaction between a user and an item, we calculate the similarity between the user vector and the item vector using the dot product. Positive samples consist of items that users have actually interacted with in the original dataset, while negative samples consist of items that users have not interacted with. Additionally, we impose a restriction to prevent the predicted values from becoming arbitrarily large. Therefore, the predictive score between user $i$ and item $j$ is defined as follows:
\begin{equation}Pr_{i,j}={\e_{final}^{(u)}}_i \cdot {\e_{longterm}^{(v)}}_j\end{equation}
And the loss function for the main task is:
\begin{equation}\mathcal{L}_r=\sum_{i=1}^{I}\sum_{k=1}^{N_{pr}}{\rm{max}}(0,1-Pr_{i,p_k}+Pr_{i,n_k})\end{equation}
where $N_{pr}$ is the number of samples, $p_k$ represents the ($k$)-th positive sample index and $n_k$ represents the ($k$)-th negative one.

\subsection{Personalized Self-augmented Learning}
While the aforementioned long and short-term structures have the ability to combine periodical higher-order collaborative and sequential information to capture dynamic user interests, sparse short-term graphs often suffer from a significant noise problem. To address this challenge, as depicted in Figure \ref{fig:ssl}, we propose a personalized self-augmented learning approach. This approach enhances the learning of user-item interactions and mitigates the impact of noise in the short term.

The rationale behind the approach is as follows: when the long-term relationship between a user and an item is weak, the interaction observed in the short term may be considered as noise. However, there are certain users who exhibit sudden short-term preferences or have highly variable preferences and interests. To cater to users with different levels of stability, it is necessary to establish varying degrees of relationship enhancement. To achieve this, we personalize the self-augmented learning component.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.44\textwidth]{figure/self-augmented-learning.pdf}
    \caption{Workflow of the self-augmented learning.}
    \label{fig:ssl}
\end{figure}

For every short-term period, we randomly select an edge $D_{t, i,j}$ composed of node user $i$ and node item $j$ and the corresponding edge $\hat{D}_{i,j}$ which is composed of node $i$ and node $j$ in the long-term feature space. $V^\sk_{t, i,j}$ is the value of edge $D_{t, i,j}$ and $V^\sh_{i,j}$ is the value of long-term edge $\hat{D}_{i,j}$. $V^\sk_{t, i,j}$ and $V^\sh_{i,j}$ are defined as scalar values calculated by the Hadamard product, the non-linear activation function and the summation dimensionality reduction:
\begin{equation}\mathbf{V}^\sk_{t,i,j}'=\sigma({\e^{(u)}_{t}}_{i}\odot{\e_{t}^{(v)}}_{j}),V^\sk_{t,i,j}=\sum_{k=1}^d {\mathbf{V}^\sk_{t,i,j}'}_k\end{equation}
\begin{equation}\mathbf{V}^\sh_{i,j}'=\sigma({\e_{longterm}^{(u)}}_{i}\odot{\e_{longterm}^{(v)}}_{j}), V^\sh_{i,j}=\sum_{k=1}^d {\mathbf{V}^\sh_{i,j}'}_k\end{equation}

This implies that a higher edge value indicates a stronger correlation between nodes $i$ and $j$. We then randomly select edges involving other nodes $i'$ and $j'$ for comparison. In our objective function, if $V^\sh_{i,j}$ is greater than $V^\sh_{i',j'}$, it signifies a higher long-term correlation between node $i$ and node $j$, while node $i'$ has a weaker relationship with node $j'$. Optimizing the objective function will increase the short-term correlation between node $i$ and node $j$, while reducing the correlation between node $i'$ and node $j'$. The loss function is shown as follows:
\begin{equation}\mathcal{L}_{sal}=\sum_{t=1}^T\sum_{k=1}^{N_{sal}}{\rm{max}}(0,1-(w^{(u)}_{t,i_k}V^\sh_{i_k,j_k}-w^{(u)}_{t,i'_k}V^\sh_{i'_k,j'_k})\cdot(V^\sk_{t,i_k,j_k}-V^\sk_{t,i'_k,j'_k}))\label{sal}\end{equation}
where $N_{sal}$ is the number of sample pairs in every period in our personalized self-augmented learning task, meanwhile, every sample pair is denoted as $\langle (i_k,j_k), (i'_k,j'_k) \rangle$.

For the personalized component, in order to obtain a weight $w^{(u)}_{t}$ that represents the stability of a user in different periods, we employ multi-layer perceptrons to assess the disparity between the long-term and short-term embeddings of a user:
\begin{equation}\mathbf{\Gamma}_{t,i}={\sigma}(({\e_{longterm}^{(u)}}_{i}+{\e^{(u)}_{t}}_{i}+{\e_{longterm}^{(u)}}_{i}\odot{\e^{(u)}_{t}}_{i})\mathbf{W}_1+\mathbf{b}_1)\end{equation}
\begin{equation}w^{(u)}_{t,i}=\Phi(\mathbf{\Gamma}_{t,i}\mathbf{W}_2+b_2)\end{equation}
where $\mathbf{W}_1 \in \mathbb{R}^{d\times d_{sal}}$, $\mathbf{W}_2 \in \mathbb{R}^{d_{sal} \times 1}$, $\mathbf{b}_1 \in \mathbb{R}^{d_{sal}}$, and $b_2 \in \mathbf{R}$ are trainable parameters used for feature transformation. The weight $w^{(u)}_{t, i}$ determines the credibility of the long-term edge value as a reference for noise correction in the ($t$)-th period, with a larger weight indicating higher credibility.

Lastly, we exclude the backpropagation of the long-term edge values $V^\sh_{i,j}$ and $V^\sh_{i',j'}$, directing the optimization process towards correcting the short-term edge values.

Conclusively, we integrate our self-augmented loss with our main task prediction loss into a unified objective:
\begin{equation}\mathcal{L}=\mathcal{L}_r+\lambda_1\cdot \mathcal{L}_{sal} + \lambda_2 \cdot {\left\| \Theta \right\|}^2_{\rm{F}}\end{equation}

We minimize the loss function $\mathcal{L}$ using the Adam optimizer. The weights $\lambda_1$ and $\lambda_2$ are used to balance the importance of different loss terms. Additionally, we apply weight decay with $l_2$ regularization on the parameters $\Theta$ of our model.

\subsection{In-Depth Analysis of \model }
\subsubsection{\bf Theoretical Analysis of \model}
Our personalized SAL architecture addresses short-term noise by generating adaptive gradients based on users who exhibit significant disparities between their long-term and short-term preferences. More specifically, for Eq. \eqref{sal}, we can quantify the impact of $\hat{D}_{i,j},{D}_{i,j},\hat{D}_{i',j'},{D}_{i',j'}$ on the learned embeddings as follows:
\begin{align}
&c'(w^{(u)}_{t,i'})=V^\sh_{i',j'}\cdot(V^\sk_{t,i,j}-V^\sk_{t,i',j'})=V^\sh_{i',j'}V^\sk_{t,i,j}-V^\sh_{i',j'}V^\sk_{t,i',j'}\notag\\
&c'(w^{(u)}_{t,i})=V^\sh_{i,j}\cdot(V^\sk_{t,i',j'}-V^\sk_{t,i,j})=V^\sh_{i,j}V^\sk_{t,i',j'}-V^\sh_{i,j}V^\sk_{t,i,j}
\label{w}
\end{align}
\begin{align}
c'(V^\sk_{t,i',j'})=w^{(u)}_{t,i}V^\sh_{i,j}-w^{(u)}_{t,i'}V^\sh_{i',j'}\notag\\
c'(V^\sk_{t,i,j})=w^{(u)}_{t,i'}V^\sh_{i',j'}-w^{(u)}_{t,i}V^\sh_{i,j}\label{S}
\end{align}
where $c'(x)$ represents the gradient with respect to $x$. In Eq. \eqref{w}, if $V^\sk_{t,i,j}-V^\sk_{t,i',j'}>0$, the gradient $c'(w^{(u)}_{t,i'})$ will monotonically increase with the variation of $V^\sh_{i',j'}$. Moreover, when the difference between the long-term value and short-term edge value is larger, \ie, when $V^\sh_{i',j'} V^\sk_{t, i',j'}$ is smaller, the learning gradient of $w^{(u)}_{t, i'}$ will be larger. The same applies to the effect of $V^\sh_{i,j}$ and $V^\sk_{t,i,j}$ on the gradient of $w^{(u)}_{t,i}$. In Eq. \eqref{S}, if $w^{(u)}_{t, i'}V^\sh_{i',j'}$ is small, indicating that user $i'$ exhibits unstable short-term behavior and has a weak long-term relationship with item $j'$, the gradient of $V^\sk_{t, i',j'}$ will increase. Overall, self-augmented learning emphasizes gradients from samples with instability between long-term and short-term user-item relationships, thereby enhancing the model training process.


Furthermore, we partition the long-term graph into multiple short-term graphs, which allows us to focus on the short-term features individually. This approach introduces a new level of granularity for capturing user preferences, in addition to the global graph level and user behavior sequence level. By leveraging this fine-grained information, our model can learn novel insights and achieve improved recommendation performance.

%\subsubsection{\bf Model Complexity Analyses}
%We put it in Appendix.
